DarkBERT: A Language Model for the Dark Side of the Internet

Recent research has suggested that there are clear differences in the language used in the Dark Web compared to that of the Surface Web. As studies on the Dark Web commonly require textual analysis of the domain, language models specific to the Dark Web may provide valuable insights to researchers. In this work, we introduce DarkBERT, a language model pretrained on Dark Web data. We describe the steps taken to filter and compile the text data used to train DarkBERT to combat the extreme lexical and structural diversity of the Dark Web that may be detrimental to building a proper representation of the domain. We evaluate DarkBERT and its vanilla counterpart along with other widely used language models to validate the benefits that a Dark Web domain specific model offers in various use cases. Our evaluations show that DarkBERT outperforms current language models and may serve as a valuable resource for future research on the Dark Web.

==> section/background.tex <==
\section{Background: The Dark Web}
\label{sec:background}

%\note{(this unindexed part of the Internet is also known as the \textit{Deep Web}~\footnote{Not to be confused with the \textit{Dark Web}. \textit{Deep Web} and \textit{Dark Web} are somewhat misused interchangeably in media, but in this paper we refer to the Dark Web as a subset of the Deep Web that is inaccessible through standard web browsers.}. Conversely, the portion of the Internet indexed by search engines is usually referred to as the \textit{Surface Web})}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figure/darkbert_overview.pdf}
    \caption{Illustration of the DarkBERT pretraining process and the various use case scenarios for evaluation.}
    \label{fig:darkbert}
\end{figure*}

%The \textit{Dark Web} can generally be defined as a subset of the Internet that is not indexed by web search engines such as Google \textit{and} is inaccessible through a standard web browser. Conversely, the portion of the Internet indexed by search engines is usually referred to as the \textit{Surface Web}. To access the Dark Web, specialized overlay network applications such as Tor (The Onion Router)~\cite{tor-269582} are required. Tor also hosts \textit{hidden services} (\textit{onion services}) --- TCP services that run inside its network to achieve a two-way anonymity in which the client and the server IP addresses are hidden from each other~\cite{biryukov-torhiddenservice}.

This sense of identity obscurity provided to the Dark Web users comes with a catch; many of the underground activities prevalent in the Dark Web are immoral/illegal in nature, ranging from content hosting such as data leaks to drug sales~\cite{al-nabki-etal-2017-classifying, coda_naacl2022}. The popularity of the Dark Web as a platform of choice for malicious activities has garnered interest from researchers and security experts alike.

%Another characteristic of the Dark Web is that many of the pages contain nearly identical or duplicate content due to the availability of free hosting services on the onion domain~\cite{ALNABKI2019212}. The abundance of cloned websites can be attributed to illegal services~\cite{doppelgangers-www2019}. This is especially evident as hidden services are generally ephemeral --- more than half of the pages in the onion domains disappear within the first 24 hours since publication~\cite{OWENSON201817}. As some illegal activities in the Dark Web require interaction from customers or even potential victims such as phishing websites~\cite{doppelgangers-www2019}, it is advantageous for malicious users to create and host multiple copies of pages to increase visibility.

%\subsection{Domain-Specific Language Models}
%\label{sec:bg-language-models}

%A significant progress in research was made in the natural language processing (NLP) community with the introduction of deep neural language models that are capable of capturing context in lengthy texts~\cite{mikolov-rnn, peters-etal-2018-deep}. 
%The idea of pretraining models through the use of large text datasets has shown to achieve state-of-the-art results through task-specific fine-tuning, highlighting the potential of pretrained language models as a key factor in NLP tasks~\cite{NEURIPS2020_lm_fewshot, peters-etal-2018-deep, qiu2020pre}. The success of pretrained language models like BERT~\cite{devlin-etal-2019-bert} has given rise to language models which are pretrained using domain-specific data. 
%Domain-specific adaptations of pretrained language models have shown promising results for domain-specific tasks~\cite{biobert-paper, chalkidis-etal-2020-legalbert, beltagy-etal-2019-scibert}. The effectiveness shown by such domain-specific pretrained language models suggests that an adaptation to the Dark Web domain may bring potential as a suitable NLP tool for Dark Web analysis.


%Further advancements were made with the Transformer architecture~\cite{attention-is-all-you-need} which allowed for better long-range dependency modeling~\cite{transformer-survey} while enabling faster computation through parallelizable layers~\cite{attention-is-all-you-need}, and was incorporated in language models such as GPT~\cite{radford2018improving} and BERT~\cite{devlin-etal-2019-bert}. 

%BERT in particular is known for its use of the masked language model (MLM) objective, which randomly masks words in the input sentence for the model to correctly predict the original word using surrounding context. In order to understand sentence relationships, BERT also uses next sentence prediction (NSP) task in which the model is given two sentences (one is the correct next sentence and the other is a random sentence from the text corpus) to choose from during pretraining.

%Variants of BERT have surfaced shortly after, addressing some of the issues that the original architecture faced such as the massive number of parameters that make the model hard to train using limited GPU/TPU memory~\cite{albert}, or questioning the design choices of BERT such as the actual necessity of the NSP task for pretraining~\cite{roberta-paper, NEURIPS2019_XLNET}. One of the variants called RoBERTa~\cite{roberta-paper} demonstrated that the NSP task is not particularly useful for improving downstream task performance and opted to use only the MLM objective during pretraining. RoBERTa also uses a \textit{dynamic masking} approach in which the masking patterns are generated each time a sequence is fed to the model. This is in contrast to the \textit{static masking} approach in BERT, where the training data is duplicated 10 times and masking is applied only once during text processing. The above design changes made by RoBERTa along with a larger pretraining text corpus and hyperparameter tweaks allow the model to achieve better performance compared to BERT~\cite{roberta-paper}. 


==> section/discussion.tex <==
\section{Discussion}
\label{discussion}
Discussion goes here.

==> table/darkweb-data-cat-final.tex <==
\begin{table}[t]
\centering
\caption{Statistics for the pretraining corpus used for DarkBERT.}
\label{tab:darkweb-data-cat-final}
\resizebox{\columnwidth}{!}{%
  \begin{tabular}{lrcrr}
    \toprule
    Category & Page Count & Total Size & Deduplication Rate & Total Reduction Rate \\
    \midrule
    Pornography & 224,781 & 971.0 MB & 2.91\% & 89.98\% \\
    Drugs & 228,965 & 766.7 MB & 23.31\% & 56.19\% \\
    Financial & 253,171 & 874.1 MB & 12.45\% & 58.38\%\\
    Gambling & 40,584 & 137.5 MB & 5.37\% & 5.37\%\\
    Cryptocurrency & 249,811 & 897.6 MB & 10.28\% & 34.00\%\\
    Hacking & 57,183 & 242.7 MB & 75.73\% & 93.09\%\\
    Arms / Weapons & 43,250 & 129.9 MB & 6.15\% & 6.15\%\\
    Violence & 253,566 & 959.8 MB & 4.02\% & 20.68\%\\
    Electronics & 381,218 & 850.4 MB & 4.17\% & 4.45\%\\
    \midrule
    Total & 1,732,529 & 5.83 GB & 18.69\% & 71.96\%\\
  \bottomrule
\end{tabular}%
}
\end{table}

==> table/darkweb-data-category.tex <==
\begin{table}[t]
\centering
\caption{Dark Web data page classification statistics.}
\label{tab:darkweb-data-category}
\resizebox{\columnwidth}{!}{%
  \begin{tabular}{lrcc}
    \toprule
    Category & Page Count & Total Size (in GB) & Average Size per Page (in KB)\\
    \midrule
    Pornography & 2,267,628 & 9.70 GB & 4.28 KB \\
    Drugs & 503,433 & 1.75 GB & 3.47 KB \\
    Financial & 637,917 & 2.10 GB & 3.29 KB\\
    Gambling & 43,041 & 0.15 GB & 3.38 KB\\
    Cryptocurrency & 412,349 & 1.36 GB & 3.29 KB\\
    Hacking & 801,330 & 3.51 GB & 4.38 KB\\
    Arms / Weapons & 46,616 & 0.14 GB & 2.70 KB\\
    Violence & 323,738 & 1.21 GB & 3.74 KB\\
    Electronics & 401,196 & 0.89 GB & 2.21 KB\\
    \midrule
    Total & 5,437,248 & 20.79 GB & -\\
  \bottomrule
\end{tabular}%
}
\end{table}
